Brief announcement: A special case of maximum flow over time with network changes

We consider the problem of finding the value of a maximum flow over time in a network with uniform edge lengths where the edge capacities change at specific time instants. To solve this problem, we show how to construct a condensed version of a Time Expanded Network (cTEN) whose standard max flow value is the same as the max flow over time on the original network. In particular, for a graph with $n$ nodes, $m$ edges, and $\mu$ {\em critical times} where some edge capacity changes, we obtain a cTEN with $O(n^2\mu)$ nodes and $O(\mu mn)$ edges. This implies that the problem can be solved in $O(\mu^2n^3m)$ time using the combinatorial max flow algorithm of Orlin [Orl13], or in $O(\mu^{(1+o(1))}(nm)^{1+o(1)}\log (UT))$ time using the algorithm of Chen et al. [CKL+22], where $U$ is the maximum capacity of any edge and $T$ is the time horizon. We focus on graphs that experience many time changes across the period of interest, as in such graphs the $\mu$ term dominates the runtime.

==> figures/bad_edge_in.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp7161090055125632] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (273,144.5) .. controls (273,139.81) and (276.81,136) .. (281.5,136) .. controls (286.19,136) and (290,139.81) .. (290,144.5) .. controls (290,149.19) and (286.19,153) .. (281.5,153) .. controls (276.81,153) and (273,149.19) .. (273,144.5) -- cycle ;
%Shape: Circle [id:dp2785682741455575] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (273,104.5) .. controls (273,99.81) and (276.81,96) .. (281.5,96) .. controls (286.19,96) and (290,99.81) .. (290,104.5) .. controls (290,109.19) and (286.19,113) .. (281.5,113) .. controls (276.81,113) and (273,109.19) .. (273,104.5) -- cycle ;
%Shape: Circle [id:dp19076284805310428] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (273,64.5) .. controls (273,59.81) and (276.81,56) .. (281.5,56) .. controls (286.19,56) and (290,59.81) .. (290,64.5) .. controls (290,69.19) and (286.19,73) .. (281.5,73) .. controls (276.81,73) and (273,69.19) .. (273,64.5) -- cycle ;
%Shape: Circle [id:dp9092256572451831] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (273,24.5) .. controls (273,19.81) and (276.81,16) .. (281.5,16) .. controls (286.19,16) and (290,19.81) .. (290,24.5) .. controls (290,29.19) and (286.19,33) .. (281.5,33) .. controls (276.81,33) and (273,29.19) .. (273,24.5) -- cycle ;
%Shape: Circle [id:dp683293517204052] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (349,144.5) .. controls (349,139.81) and (352.81,136) .. (357.5,136) .. controls (362.19,136) and (366,139.81) .. (366,144.5) .. controls (366,149.19) and (362.19,153) .. (357.5,153) .. controls (352.81,153) and (349,149.19) .. (349,144.5) -- cycle ;
%Shape: Circle [id:dp45594825716117193] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (349,104.5) .. controls (349,99.81) and (352.81,96) .. (357.5,96) .. controls (362.19,96) and (366,99.81) .. (366,104.5) .. controls (366,109.19) and (362.19,113) .. (357.5,113) .. controls (352.81,113) and (349,109.19) .. (349,104.5) -- cycle ;
%Shape: Circle [id:dp977301255052822] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (349,64.5) .. controls (349,59.81) and (352.81,56) .. (357.5,56) .. controls (362.19,56) and (366,59.81) .. (366,64.5) .. controls (366,69.19) and (362.19,73) .. (357.5,73) .. controls (352.81,73) and (349,69.19) .. (349,64.5) -- cycle ;
%Shape: Circle [id:dp7519315848908104] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (349,24.5) .. controls (349,19.81) and (352.81,16) .. (357.5,16) .. controls (362.19,16) and (366,19.81) .. (366,24.5) .. controls (366,29.19) and (362.19,33) .. (357.5,33) .. controls (352.81,33) and (349,29.19) .. (349,24.5) -- cycle ;
%Straight Lines [id:da8798551389205505] 
\draw    (281.5,136) -- (281.5,115) ;
\draw [shift={(281.5,113)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7433959986367038] 
\draw    (281.5,96) -- (281.5,75) ;
\draw [shift={(281.5,73)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3951267275664734] 
\draw    (281.5,56) -- (281.5,35) ;
\draw [shift={(281.5,33)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7743748563029189] 
\draw    (357.5,56) -- (357.5,35) ;
\draw [shift={(357.5,33)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da18891782466166385] 
\draw    (357.5,96) -- (357.5,75) ;
\draw [shift={(357.5,73)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2856568988667145] 
\draw    (357.5,136) -- (357.5,115) ;
\draw [shift={(357.5,113)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7223338790186591] 
\draw    (290,64.5) -- (347.34,25.62) ;
\draw [shift={(349,24.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8206448722041872] 
\draw    (290,104.5) -- (347.34,65.62) ;
\draw [shift={(349,64.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8540782557611089] 
\draw    (290,144.5) -- (347.34,105.62) ;
\draw [shift={(349,104.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8061929970122705] 
\draw [line width=3]    (237.33,127) -- (174.14,180.76) ;
\draw [shift={(170.33,184)}, rotate = 319.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=3]    (20.77,-6.25) .. controls (13.2,-2.65) and (6.28,-0.57) .. (0,0) .. controls (6.28,0.57) and (13.2,2.66) .. (20.77,6.25)   ;
%Straight Lines [id:da4871105899673476] 
\draw [line width=3]    (393.33,129) -- (450.65,181.62) ;
\draw [shift={(454.33,185)}, rotate = 222.55] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=3]    (20.77,-6.25) .. controls (13.2,-2.65) and (6.28,-0.57) .. (0,0) .. controls (6.28,0.57) and (13.2,2.66) .. (20.77,6.25)   ;
%Shape: Circle [id:dp5729003103773256] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,241.5) .. controls (39,236.81) and (42.81,233) .. (47.5,233) .. controls (52.19,233) and (56,236.81) .. (56,241.5) .. controls (56,246.19) and (52.19,250) .. (47.5,250) .. controls (42.81,250) and (39,246.19) .. (39,241.5) -- cycle ;
%Shape: Circle [id:dp5373229270759778] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,201.5) .. controls (39,196.81) and (42.81,193) .. (47.5,193) .. controls (52.19,193) and (56,196.81) .. (56,201.5) .. controls (56,206.19) and (52.19,210) .. (47.5,210) .. controls (42.81,210) and (39,206.19) .. (39,201.5) -- cycle ;
%Shape: Circle [id:dp842596149334061] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,161.5) .. controls (39,156.81) and (42.81,153) .. (47.5,153) .. controls (52.19,153) and (56,156.81) .. (56,161.5) .. controls (56,166.19) and (52.19,170) .. (47.5,170) .. controls (42.81,170) and (39,166.19) .. (39,161.5) -- cycle ;
%Shape: Circle [id:dp8348578864253071] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,121.5) .. controls (39,116.81) and (42.81,113) .. (47.5,113) .. controls (52.19,113) and (56,116.81) .. (56,121.5) .. controls (56,126.19) and (52.19,130) .. (47.5,130) .. controls (42.81,130) and (39,126.19) .. (39,121.5) -- cycle ;
%Shape: Circle [id:dp4642192669458418] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (115,241.5) .. controls (115,236.81) and (118.81,233) .. (123.5,233) .. controls (128.19,233) and (132,236.81) .. (132,241.5) .. controls (132,246.19) and (128.19,250) .. (123.5,250) .. controls (118.81,250) and (115,246.19) .. (115,241.5) -- cycle ;
%Shape: Circle [id:dp2424321908010072] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (115,201.5) .. controls (115,196.81) and (118.81,193) .. (123.5,193) .. controls (128.19,193) and (132,196.81) .. (132,201.5) .. controls (132,206.19) and (128.19,210) .. (123.5,210) .. controls (118.81,210) and (115,206.19) .. (115,201.5) -- cycle ;
%Shape: Circle [id:dp9531236566705756] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (115,161.5) .. controls (115,156.81) and (118.81,153) .. (123.5,153) .. controls (128.19,153) and (132,156.81) .. (132,161.5) .. controls (132,166.19) and (128.19,170) .. (123.5,170) .. controls (118.81,170) and (115,166.19) .. (115,161.5) -- cycle ;
%Shape: Circle [id:dp2368160418418439] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (115,121.5) .. controls (115,116.81) and (118.81,113) .. (123.5,113) .. controls (128.19,113) and (132,116.81) .. (132,121.5) .. controls (132,126.19) and (128.19,130) .. (123.5,130) .. controls (118.81,130) and (115,126.19) .. (115,121.5) -- cycle ;
%Straight Lines [id:da3870608417603054] 
\draw    (47.5,233) -- (47.5,212) ;
\draw [shift={(47.5,210)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da06605974555890248] 
\draw    (47.5,193) -- (47.5,172) ;
\draw [shift={(47.5,170)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da697114319324198] 
\draw    (47.5,153) -- (47.5,132) ;
\draw [shift={(47.5,130)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da24921662981005888] 
\draw    (123.5,153) -- (123.5,132) ;
\draw [shift={(123.5,130)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da19371983230920664] 
\draw    (123.5,193) -- (123.5,172) ;
\draw [shift={(123.5,170)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da01469946540676026] 
\draw    (123.5,233) -- (123.5,212) ;
\draw [shift={(123.5,210)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8451969896648979] 
\draw    (56,161.5) -- (113.34,122.62) ;
\draw [shift={(115,121.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4488597636527243] 
\draw    (56,201.5) -- (113.34,162.62) ;
\draw [shift={(115,161.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da38331827921477357] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (56,241.5) -- (111.69,203.74) ;
\draw [shift={(115,201.5)}, rotate = 145.86] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Shape: Circle [id:dp6619625956504198] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (513,247.5) .. controls (513,242.81) and (516.81,239) .. (521.5,239) .. controls (526.19,239) and (530,242.81) .. (530,247.5) .. controls (530,252.19) and (526.19,256) .. (521.5,256) .. controls (516.81,256) and (513,252.19) .. (513,247.5) -- cycle ;
%Shape: Circle [id:dp0033014768550638784] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (513,207.5) .. controls (513,202.81) and (516.81,199) .. (521.5,199) .. controls (526.19,199) and (530,202.81) .. (530,207.5) .. controls (530,212.19) and (526.19,216) .. (521.5,216) .. controls (516.81,216) and (513,212.19) .. (513,207.5) -- cycle ;
%Shape: Circle [id:dp667814613952133] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (513,167.5) .. controls (513,162.81) and (516.81,159) .. (521.5,159) .. controls (526.19,159) and (530,162.81) .. (530,167.5) .. controls (530,172.19) and (526.19,176) .. (521.5,176) .. controls (516.81,176) and (513,172.19) .. (513,167.5) -- cycle ;
%Shape: Circle [id:dp2515532869295318] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (513,127.5) .. controls (513,122.81) and (516.81,119) .. (521.5,119) .. controls (526.19,119) and (530,122.81) .. (530,127.5) .. controls (530,132.19) and (526.19,136) .. (521.5,136) .. controls (516.81,136) and (513,132.19) .. (513,127.5) -- cycle ;
%Shape: Circle [id:dp9641022814306601] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (589,247.5) .. controls (589,242.81) and (592.81,239) .. (597.5,239) .. controls (602.19,239) and (606,242.81) .. (606,247.5) .. controls (606,252.19) and (602.19,256) .. (597.5,256) .. controls (592.81,256) and (589,252.19) .. (589,247.5) -- cycle ;
%Shape: Circle [id:dp056768503103014734] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (589,207.5) .. controls (589,202.81) and (592.81,199) .. (597.5,199) .. controls (602.19,199) and (606,202.81) .. (606,207.5) .. controls (606,212.19) and (602.19,216) .. (597.5,216) .. controls (592.81,216) and (589,212.19) .. (589,207.5) -- cycle ;
%Shape: Circle [id:dp8917433154097076] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (589,167.5) .. controls (589,162.81) and (592.81,159) .. (597.5,159) .. controls (602.19,159) and (606,162.81) .. (606,167.5) .. controls (606,172.19) and (602.19,176) .. (597.5,176) .. controls (592.81,176) and (589,172.19) .. (589,167.5) -- cycle ;
%Shape: Circle [id:dp18404898320394802] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (589,127.5) .. controls (589,122.81) and (592.81,119) .. (597.5,119) .. controls (602.19,119) and (606,122.81) .. (606,127.5) .. controls (606,132.19) and (602.19,136) .. (597.5,136) .. controls (592.81,136) and (589,132.19) .. (589,127.5) -- cycle ;
%Straight Lines [id:da735644395943005] 
\draw    (521.5,239) -- (521.5,218) ;
\draw [shift={(521.5,216)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9021864485605136] 
\draw    (521.5,199) -- (521.5,178) ;
\draw [shift={(521.5,176)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4252828613279789] 
\draw    (521.5,159) -- (521.5,138) ;
\draw [shift={(521.5,136)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5883529319925151] 
\draw    (597.5,159) -- (597.5,138) ;
\draw [shift={(597.5,136)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8502110410009398] 
\draw    (597.5,199) -- (597.5,178) ;
\draw [shift={(597.5,176)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6068303381912192] 
\draw    (597.5,239) -- (597.5,218) ;
\draw [shift={(597.5,216)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da792652670332683] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (530,167.5) -- (587.34,128.62) ;
\draw [shift={(589,127.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4202254089209285] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (530,207.5) -- (585.69,169.74) ;
\draw [shift={(589,167.5)}, rotate = 145.86] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Straight Lines [id:da6010276342932435] 
\draw    (530,247.5) -- (587.34,208.62) ;
\draw [shift={(589,207.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (248,167) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle i\in C$};
% Text Node
\draw (342,166) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle j\in V\setminus C$};
% Text Node
\draw (14,264) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle i\in C$};
% Text Node
\draw (108,263) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle j\in V\setminus C$};
% Text Node
\draw (488,270) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle i\in C$};
% Text Node
\draw (582,269) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle j\in V\setminus C$};
% Text Node
\draw (182,114) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi _{C}^{-}$};
% Text Node
\draw (429,119) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi _{C}^{+}$};
% Text Node
\draw (377,54) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi ( j)$};
% Text Node
\draw (242.33,95) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi ( i)$};
% Text Node
\draw (23,25.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Huge (a)}};


\end{tikzpicture}


==> figures/bad_edge_out.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp7932995658850512] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (273,144.5) .. controls (273,139.81) and (276.81,136) .. (281.5,136) .. controls (286.19,136) and (290,139.81) .. (290,144.5) .. controls (290,149.19) and (286.19,153) .. (281.5,153) .. controls (276.81,153) and (273,149.19) .. (273,144.5) -- cycle ;
%Shape: Circle [id:dp0034500130163135356] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (273,104.5) .. controls (273,99.81) and (276.81,96) .. (281.5,96) .. controls (286.19,96) and (290,99.81) .. (290,104.5) .. controls (290,109.19) and (286.19,113) .. (281.5,113) .. controls (276.81,113) and (273,109.19) .. (273,104.5) -- cycle ;
%Shape: Circle [id:dp25797778833117024] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (273,64.5) .. controls (273,59.81) and (276.81,56) .. (281.5,56) .. controls (286.19,56) and (290,59.81) .. (290,64.5) .. controls (290,69.19) and (286.19,73) .. (281.5,73) .. controls (276.81,73) and (273,69.19) .. (273,64.5) -- cycle ;
%Shape: Circle [id:dp6098747098736959] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (273,24.5) .. controls (273,19.81) and (276.81,16) .. (281.5,16) .. controls (286.19,16) and (290,19.81) .. (290,24.5) .. controls (290,29.19) and (286.19,33) .. (281.5,33) .. controls (276.81,33) and (273,29.19) .. (273,24.5) -- cycle ;
%Shape: Circle [id:dp8872814462791174] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (349,144.5) .. controls (349,139.81) and (352.81,136) .. (357.5,136) .. controls (362.19,136) and (366,139.81) .. (366,144.5) .. controls (366,149.19) and (362.19,153) .. (357.5,153) .. controls (352.81,153) and (349,149.19) .. (349,144.5) -- cycle ;
%Shape: Circle [id:dp18912629011712223] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (349,104.5) .. controls (349,99.81) and (352.81,96) .. (357.5,96) .. controls (362.19,96) and (366,99.81) .. (366,104.5) .. controls (366,109.19) and (362.19,113) .. (357.5,113) .. controls (352.81,113) and (349,109.19) .. (349,104.5) -- cycle ;
%Shape: Circle [id:dp27013857216263926] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (349,64.5) .. controls (349,59.81) and (352.81,56) .. (357.5,56) .. controls (362.19,56) and (366,59.81) .. (366,64.5) .. controls (366,69.19) and (362.19,73) .. (357.5,73) .. controls (352.81,73) and (349,69.19) .. (349,64.5) -- cycle ;
%Shape: Circle [id:dp8590621569421468] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (349,24.5) .. controls (349,19.81) and (352.81,16) .. (357.5,16) .. controls (362.19,16) and (366,19.81) .. (366,24.5) .. controls (366,29.19) and (362.19,33) .. (357.5,33) .. controls (352.81,33) and (349,29.19) .. (349,24.5) -- cycle ;
%Straight Lines [id:da7702917288937354] 
\draw    (281.5,136) -- (281.5,115) ;
\draw [shift={(281.5,113)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da11310231787297687] 
\draw    (281.5,96) -- (281.5,75) ;
\draw [shift={(281.5,73)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7975679738021204] 
\draw    (281.5,56) -- (281.5,35) ;
\draw [shift={(281.5,33)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da16173958487075524] 
\draw    (357.5,56) -- (357.5,35) ;
\draw [shift={(357.5,33)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da42887396016240853] 
\draw    (357.5,96) -- (357.5,75) ;
\draw [shift={(357.5,73)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da896637157142876] 
\draw    (357.5,136) -- (357.5,115) ;
\draw [shift={(357.5,113)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da09346790596722654] 
\draw    (290,64.5) -- (347.34,25.62) ;
\draw [shift={(349,24.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2894438172207019] 
\draw    (290,104.5) -- (347.34,65.62) ;
\draw [shift={(349,64.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5590559034228093] 
\draw    (290,144.5) -- (347.34,105.62) ;
\draw [shift={(349,104.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da37635971915350663] 
\draw [line width=3]    (237.33,127) -- (174.14,180.76) ;
\draw [shift={(170.33,184)}, rotate = 319.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=3]    (20.77,-6.25) .. controls (13.2,-2.65) and (6.28,-0.57) .. (0,0) .. controls (6.28,0.57) and (13.2,2.66) .. (20.77,6.25)   ;
%Straight Lines [id:da6498774315631868] 
\draw [line width=3]    (393.33,129) -- (450.65,181.62) ;
\draw [shift={(454.33,185)}, rotate = 222.55] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=3]    (20.77,-6.25) .. controls (13.2,-2.65) and (6.28,-0.57) .. (0,0) .. controls (6.28,0.57) and (13.2,2.66) .. (20.77,6.25)   ;
%Shape: Circle [id:dp9194573463375566] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (39,241.5) .. controls (39,236.81) and (42.81,233) .. (47.5,233) .. controls (52.19,233) and (56,236.81) .. (56,241.5) .. controls (56,246.19) and (52.19,250) .. (47.5,250) .. controls (42.81,250) and (39,246.19) .. (39,241.5) -- cycle ;
%Shape: Circle [id:dp1968535529715829] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,201.5) .. controls (39,196.81) and (42.81,193) .. (47.5,193) .. controls (52.19,193) and (56,196.81) .. (56,201.5) .. controls (56,206.19) and (52.19,210) .. (47.5,210) .. controls (42.81,210) and (39,206.19) .. (39,201.5) -- cycle ;
%Shape: Circle [id:dp9659936643697673] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,161.5) .. controls (39,156.81) and (42.81,153) .. (47.5,153) .. controls (52.19,153) and (56,156.81) .. (56,161.5) .. controls (56,166.19) and (52.19,170) .. (47.5,170) .. controls (42.81,170) and (39,166.19) .. (39,161.5) -- cycle ;
%Shape: Circle [id:dp5465746292676454] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (39,121.5) .. controls (39,116.81) and (42.81,113) .. (47.5,113) .. controls (52.19,113) and (56,116.81) .. (56,121.5) .. controls (56,126.19) and (52.19,130) .. (47.5,130) .. controls (42.81,130) and (39,126.19) .. (39,121.5) -- cycle ;
%Shape: Circle [id:dp24567058787845175] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (115,241.5) .. controls (115,236.81) and (118.81,233) .. (123.5,233) .. controls (128.19,233) and (132,236.81) .. (132,241.5) .. controls (132,246.19) and (128.19,250) .. (123.5,250) .. controls (118.81,250) and (115,246.19) .. (115,241.5) -- cycle ;
%Shape: Circle [id:dp508190419089338] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (115,201.5) .. controls (115,196.81) and (118.81,193) .. (123.5,193) .. controls (128.19,193) and (132,196.81) .. (132,201.5) .. controls (132,206.19) and (128.19,210) .. (123.5,210) .. controls (118.81,210) and (115,206.19) .. (115,201.5) -- cycle ;
%Shape: Circle [id:dp30388020780771763] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (115,161.5) .. controls (115,156.81) and (118.81,153) .. (123.5,153) .. controls (128.19,153) and (132,156.81) .. (132,161.5) .. controls (132,166.19) and (128.19,170) .. (123.5,170) .. controls (118.81,170) and (115,166.19) .. (115,161.5) -- cycle ;
%Shape: Circle [id:dp5118184447441998] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (115,121.5) .. controls (115,116.81) and (118.81,113) .. (123.5,113) .. controls (128.19,113) and (132,116.81) .. (132,121.5) .. controls (132,126.19) and (128.19,130) .. (123.5,130) .. controls (118.81,130) and (115,126.19) .. (115,121.5) -- cycle ;
%Straight Lines [id:da2269146390516128] 
\draw    (47.5,233) -- (47.5,212) ;
\draw [shift={(47.5,210)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da17975706936937885] 
\draw    (47.5,193) -- (47.5,172) ;
\draw [shift={(47.5,170)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7214978545225932] 
\draw    (47.5,153) -- (47.5,132) ;
\draw [shift={(47.5,130)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7727485091346127] 
\draw    (123.5,153) -- (123.5,132) ;
\draw [shift={(123.5,130)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8933904887304485] 
\draw    (123.5,193) -- (123.5,172) ;
\draw [shift={(123.5,170)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da49970357052262404] 
\draw    (123.5,233) -- (123.5,212) ;
\draw [shift={(123.5,210)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9354490582490258] 
\draw    (56,161.5) -- (113.34,122.62) ;
\draw [shift={(115,121.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8217909647895043] 
\draw    (56,201.5) -- (113.34,162.62) ;
\draw [shift={(115,161.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5826278516296206] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (56,241.5) -- (111.69,203.74) ;
\draw [shift={(115,201.5)}, rotate = 145.86] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Shape: Circle [id:dp20265699891634625] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (513,247.5) .. controls (513,242.81) and (516.81,239) .. (521.5,239) .. controls (526.19,239) and (530,242.81) .. (530,247.5) .. controls (530,252.19) and (526.19,256) .. (521.5,256) .. controls (516.81,256) and (513,252.19) .. (513,247.5) -- cycle ;
%Shape: Circle [id:dp4191334567167433] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (513,207.5) .. controls (513,202.81) and (516.81,199) .. (521.5,199) .. controls (526.19,199) and (530,202.81) .. (530,207.5) .. controls (530,212.19) and (526.19,216) .. (521.5,216) .. controls (516.81,216) and (513,212.19) .. (513,207.5) -- cycle ;
%Shape: Circle [id:dp12054458560520542] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (513,167.5) .. controls (513,162.81) and (516.81,159) .. (521.5,159) .. controls (526.19,159) and (530,162.81) .. (530,167.5) .. controls (530,172.19) and (526.19,176) .. (521.5,176) .. controls (516.81,176) and (513,172.19) .. (513,167.5) -- cycle ;
%Shape: Circle [id:dp754527176135281] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (513,127.5) .. controls (513,122.81) and (516.81,119) .. (521.5,119) .. controls (526.19,119) and (530,122.81) .. (530,127.5) .. controls (530,132.19) and (526.19,136) .. (521.5,136) .. controls (516.81,136) and (513,132.19) .. (513,127.5) -- cycle ;
%Shape: Circle [id:dp7589446444743406] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (589,247.5) .. controls (589,242.81) and (592.81,239) .. (597.5,239) .. controls (602.19,239) and (606,242.81) .. (606,247.5) .. controls (606,252.19) and (602.19,256) .. (597.5,256) .. controls (592.81,256) and (589,252.19) .. (589,247.5) -- cycle ;
%Shape: Circle [id:dp9102709192757246] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (589,207.5) .. controls (589,202.81) and (592.81,199) .. (597.5,199) .. controls (602.19,199) and (606,202.81) .. (606,207.5) .. controls (606,212.19) and (602.19,216) .. (597.5,216) .. controls (592.81,216) and (589,212.19) .. (589,207.5) -- cycle ;
%Shape: Circle [id:dp7616600886422278] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (589,167.5) .. controls (589,162.81) and (592.81,159) .. (597.5,159) .. controls (602.19,159) and (606,162.81) .. (606,167.5) .. controls (606,172.19) and (602.19,176) .. (597.5,176) .. controls (592.81,176) and (589,172.19) .. (589,167.5) -- cycle ;
%Shape: Circle [id:dp7260516370392118] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (589,127.5) .. controls (589,122.81) and (592.81,119) .. (597.5,119) .. controls (602.19,119) and (606,122.81) .. (606,127.5) .. controls (606,132.19) and (602.19,136) .. (597.5,136) .. controls (592.81,136) and (589,132.19) .. (589,127.5) -- cycle ;
%Straight Lines [id:da15677134087438493] 
\draw    (521.5,239) -- (521.5,218) ;
\draw [shift={(521.5,216)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da776504437999576] 
\draw    (521.5,199) -- (521.5,178) ;
\draw [shift={(521.5,176)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15706274233503414] 
\draw    (521.5,159) -- (521.5,138) ;
\draw [shift={(521.5,136)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5898179374699213] 
\draw    (597.5,159) -- (597.5,138) ;
\draw [shift={(597.5,136)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7883673268827551] 
\draw    (597.5,199) -- (597.5,178) ;
\draw [shift={(597.5,176)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da998418286770679] 
\draw    (597.5,239) -- (597.5,218) ;
\draw [shift={(597.5,216)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7207641074378703] 
\draw    (530,167.5) -- (587.34,128.62) ;
\draw [shift={(589,127.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da01178828073720295] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (530,207.5) -- (585.69,169.74) ;
\draw [shift={(589,167.5)}, rotate = 145.86] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Straight Lines [id:da7837170898683516] 
\draw    (530,247.5) -- (587.34,208.62) ;
\draw [shift={(589,207.5)}, rotate = 145.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (248,167) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle i\in V\setminus C$};
% Text Node
\draw (342,166) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle j\in C$};
% Text Node
\draw (14,264) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle i\in V\setminus C$};
% Text Node
\draw (108,263) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle j\in C$};
% Text Node
\draw (488,270) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle i\in V\setminus C$};
% Text Node
\draw (582,269) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle j\in C$};
% Text Node
\draw (182,114) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi _{C}^{-}$};
% Text Node
\draw (429,119) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi _{C}^{+}$};
% Text Node
\draw (377,54) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi ( j)$};
% Text Node
\draw (242.33,95) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi ( i)$};
% Text Node
\draw (31,16.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Huge (b)}};


\end{tikzpicture}


==> macros.tex <==
\usepackage[utf8]{inputenc}
\usepackage{fullpage,times}
% \usepackage[numbers]{natbib}
\usepackage{enumerate}
\usepackage[dvipsnames]{xcolor}

\newcommand{\change}[1]{{\color{Mahogany} #1}}
\newcommand{\levelval}{\eta}


%% The amsthm package provides extended theorem environments
\usepackage{amsmath,amsfonts,amsthm,amssymb,multirow,hyperref}
\usepackage{cancel} 
\usepackage{mathtools}
\usepackage[normalem]{ulem}



%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
\usepackage{lineno}
%% for the whole article with \linenumbers.
% \linenumbers


\usepackage{algorithm}
% add [noend] before this to ditch the ends
\usepackage[noend]{algpseudocode}


\usepackage{parskip} %% used to replace indents with space between paragraphs

\newcommand{\kristin}[1]{\color{blue}[{\small {\bf Kristin:} { {#1}}}]\color{black}}
\newcommand{\kristinEDIT}[2]{\textcolor{blue}{\sout{#1}{#2}}}
\newcommand{\shuchi}[1]{\color{olive}[{\small {\bf Shuchi:} { {#1}}}]\color{black}}
\newcommand{\shuchiEDIT}[2]{\textcolor{olive}{\sout{#1}{#2}}}
\newcommand{\hide}[1]{}


\newcommand\multiset[1]{\{{#1}\}}

\renewcommand\tilde{\widetilde}

% \documentclass[final,onefignum,onetabnum]{siamart190516}

%% ------------------------------------------------------------------
%% Code used in examples, needed to reproduce 
%% ------------------------------------------------------------------
%% Used for \set, used in an example below
\usepackage{braket,amsfonts}

%% Used in table example below
\usepackage{array,subcaption}

%% Used in table and figure examples below
% \usepackage[caption=false]{subfig}
%% Used for papers with subtables created with the subfig package
% \captionsetup[subtable]{position=bottom}
% \captionsetup[table]{position=bottom}

%% Used for PgfPlots example, shown in the "Figures" section below.
\usepackage{pgfplots}

%% Used for creating new theorem and remark environments

\newtheoremstyle{custom}% name
{2mm}% Space above
{2mm}% Space below
{\itshape}% Body font
{}% Indent amount
{\bfseries}% Theorem head font
{: }% Punctuation after theorem head
{0em}% Space after theorem head
{}% Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{custom}
\newcounter{names}
\counterwithin{names}{section}
\newtheorem{claim}[names]{Claim}
\newtheorem{observation}[names]{Observation}
\newtheorem{thm}[names]{Theorem}
\newtheorem{theorem}[names]{Theorem}
\newtheorem{cor}[names]{Corollary}
\newtheorem{lem}[names]{Lemma}
\newtheorem{lemma}[names]{Lemma}
\newtheorem{definition}[names]{Definition}
\newtheorem{fact}{Fact}

\newtheorem{remark}{Remark}
\newtheorem{hypothesis}{Hypothesis}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}

%% Algorithm style, could alternatively use algpseudocode
% \usepackage{algorithmic}

%% For figures
\usepackage{graphicx,epstopdf}

%% For referencing line numbers
% \Crefname{ALC@unique}{Line}{Lines}

%% For creating math operators
\usepackage{amsopn}
\DeclareMathOperator{\Range}{Range}
\DeclareMathOperator{\expect}{E}

% Stretch the pages
\patchcmd\newpage{\vfil}{}{}{}
\raggedbottom

\newcommand{\remove}[1]{}

\newenvironment{proofof}[1]{\vspace{0.1in}\noindent{\em Proof of #1.}}{\qed}


% various useful names 
\newcommand{\reals}{\mathbb{R}}
\newcommand{\perm}{\pi}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\st}{^*}
\newcommand{\decider}{b}
\newcommand{\expec}{\mathop{E}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cT}{\mathcal{T}}

\newcommand{\optflow}{F\st}
\newcommand{\getflow}{\texttt{GetFlow}}
\newcommand{\flowvalue}{\texttt{FlowValue}}
\newcommand{\findlambda}{\texttt{FindLambda}}
\newcommand{\findb}{\texttt{FindPeriod}}
\newcommand{\partflow}{\partial f}
\newcommand{\partflowrange}[2]{T_{#1}^{#2}}
\newcommand{\traveltimes}{\Gamma}
\newcommand{\moveup}[1]{\phi_{#1}^+}
\newcommand{\movedown}[1]{\phi_{#1}^-}
\newcommand{\flowbreaks}[1]{\mathcal{T}_{#1}}
\newcommand{\potentialbreaks}{\mathcal{S}}
\newcommand{\middlegap}{\texttt{MiddlePeriod}}


\newcommand{\testflow}{\lambda}
\newcommand{\verifytest}{\texttt{TestNetwork}}


\newcommand{\incl}[1]{[#1]}
\newcommand{\excl}[1]{(#1]}
\newcommand{\exclleft}[1]{[#1)}
\newcommand{\capac}{u}
\newcommand{\breaks}{\mathcal{T}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\ten}{\textsc{TEN}}
\newcommand{\cten}{\textsc{cTEN}}
\newcommand{\critcut}[1]{\textsc{Range}(#1)}
\newcommand{\critnode}[2]{\texttt{crit}_{#2}(#1)}
\newcommand{\extcrit}[1]{\texttt{extendedcrit}(#1)}
\newcommand{\critnet}[1]{\textsc{CriticalTimes}(#1)}
\newcommand{\critnetoff}[1]{\texttt{crit}\st(#1)}
\newcommand{\critset}[2]{\texttt{crit}_{#2}(#1)}
\newcommand{\critsetextra}[2]{\texttt{crit}\st_{#2}(#1)}
\newcommand{\forbidden}[3]{\texttt{forbidden}_{#1, #2}(#3)}
\newcommand{\canonqt}{\texttt{CanonicalQT}}



==> short_version/short_def.tex <==
\section{Definitions and main result}

We begin by formally defining a general version of temporal networks. Intuitively, a temporal network is parameterized by its edge capacities and lengths. 

\begin{definition}\footnote{This is not a fully general definition of a temporal network -- we restricted some of the parameters to match the assumptions of this paper and to save space.}
A time-varying, or temporal, network $N=(V,E,\tau,\{\capac_{ij}:\integers\rightarrow \reals_{\geq 0}\}_{ij\in E})$ consists of 
\begin{itemize}
    \item a set of vertices $V$,
    \item a set of directed edges $E\subseteq V\times V$, each of length $\tau$,  and
    % \item an edge length $\tau$, and
    % \item length functions $\tau$ for each edge,
    \item capacity functions $\capac_{ij}$ for each edge that denote the capacity of edges at each integral time.
    % \item node storage capacity functions $a_i$ that denote the amount of flow that can be stored at a particular node at each time step.
\end{itemize}
\end{definition}



We can now formally define flows on temporal networks. Let $\eta_{i,f}(t)$ be the net flow into $i$ at time $t$. That is, $\eta_{i,f}(t):=\sum_{j:ji\in E}\sum_{t'=0}^{t-\tau} f_{ji}(t')  -\sum_{j:ij\in E}\sum_{t'=0}^t f_{ij}(t')$. The {\em value} of flow $f$ at over time horizon $T$ is defined to be $\eta_{d,f}(T)$, where the network sink is $d$.

\begin{definition}
    An $s$-$d$ {\em flow over time $T$} in a network $(V,E,\tau,\set{\capac_{ij}})$ is a set of functions $f_{ij}:[0,T]\rightarrow \reals_{\geq 0}$ for each $ij\in E$ such that the following hold:
    \begin{enumerate}
        \item For all integers $t\in [0,T],ij\in E$, $f_{ij}(t)\leq u_{ij}(t)$ \change{(edge capacity constraint)}

         % \item For all $ij\in E$, $t+\tau>T$ or $t<0$, \change{(no flow leaves before $0$ or arrives after time $T$)}
         %    \begin{align*}
         %        f_{ij}(t)=0
         %    \end{align*}
        
        \item For all $t\in [0,T],i\in V\setminus\{s\}$: $\eta_{i,f}(t)\geq 0$
        % $0\leq \sum_{j:ji\in E}\sum_{t'=0}^{t-\tau} f_{ji}(t')  -\sum_{j:ij\in E}\sum_{t'=0}^t f_{ij}(t')$; 
        % further, equality must hold when $t=T$ and $i\in V\setminus\set{s,d}$.
        \change{(net flow into a node is always non-negative)}

        % \begin{align*}
        %     0\leq \sum_{j:ji\in E}\sum_{t'=0}^{t-\tau} f_{ji}(t')  -\sum_{j:ij\in E}\sum_{t'=0}^t f_{ij}(t') 
        % \end{align*}
       
        \item For all $i\in V\setminus\{s,d\}$: $\eta_{i,f}(T)=0,$   \change{(net flow over the whole period is $0$ for all but $s$ and $d$)}        

    \end{enumerate}


    % The {\em value} of flow $f$ at over time horizon $T$ is $\eta_{T,d,f}$. 
    % the net flow into $d$ at time $T$, which is $|f|_{T}:=\sum_{j:jd\in E}\sum_{t=0}^{T-\tau_{jd}} f_{jd}(t)  -\sum_{j:dj\in E}\sum_{t=0}^T f_{dj}(t).$
        %  \begin{align*}
        %     |f|_{T}:=\sum_{j:jd\in E}\sum_{t=0}^{T-\tau_{jd}} f_{jd}(t)  -\sum_{j:dj\in E}\sum_{t=0}^T f_{dj}(t).
        % \end{align*}
    % When $T$ is clear from context, we may write $|f|$ instead of $|f|_T$.
\end{definition}


\subsection*{Time Extended Networks (TENs)}

The classical flows  originally defined by Ford and Fulkerson \cite{ford1956} (referred to as steady-state flows in this paper) have been extensively studied, so we focus on a translation of flow over time problems on temporal networks to steady-state flow problems. The most basic way to relate these two problems is using a Time Extended Network of the temporal network $N$, which we denote as $\ten(N)$. Specifically, $\ten(N,T)$ has as its vertex set $V\times [0,T]$, and there is an edge from $(i,t)$ to $(j,t')$ of capacity $u_{ij}(t)$ for $i\neq j$ if and only if $ij\in E$ and $t'=t+\tau$. For all $i,t<T$, there is also an edge of infinite capacity from $(i,t)$ to $(i,t+1)$. The source and sink of this network are $(s,0)$ and $(d,T)$, respectively.


% \begin{definition}
% For a network $N=(V,E,\set{\tau_{ij}},\set{u_{ij}})$, source $s$, sink $d$, and time horizon $T$ we define $\ten(N,T)$ as a classical (steady-state) flow network $G$ with the following characteristics:
% \begin{itemize}
%     \item The vertex set is $V'=V\times [0,T]$.
%     \item There is an edge from $(i,t)$ to $(j,t')$ for $i\neq j$ if and only if $ij\in E$, $t'=t+\tau_{ij}$, and $u_{ij}(t)\neq 0$. Further, the capacity of this edge is $u_{ij}(t)$.
%     \item For all $i$ and all $t\in [0,T-1]$, there is an edge from $(i,t)$ to $(i,t+1)$ with infinite capacity.
%     \item The source is $(s,0)$ and the sink is $(d,T)$.
% \end{itemize}

% If $T$ is clear from context, we may just write $\ten(N)$.
% \end{definition}


For any $s,d$ and any $T$, the maximum $s$-$d$ flow over time value in $N$ is the same as the maximum steady-state $(s,0)$-$(d,T)$ flow in $\ten(N,T)$ \cite{anderson}. Thus, one solution to this problem is to run any steady-state max flow algorithm on $\ten(N,T)$.
However, the size of $\ten(N,T)$ blows up with the value of $T$, so just writing it down could take time exponential in the size of the description of $N$ and $T$. 
To exploit the succinct structure of our networks (that is, the structure of networks with piecewise constant capacities), we define a refined version of $\ten(N,T)$, which we call a {\em condensed time extended network}, or $\cten(N,A,T)$ (where $A\subseteq[0,T]$ is a set to be defined). The idea of $\cten(N,A,T)$
 is that $A$ will partition $[0,T]$ into intervals such that each interval begins at some time in $A$.
 
\begin{definition}
If $N=(V,E,\set{\tau_{ij}},\set{u_{ij}})$ is a temporal network with source $s$ and sink $d$ and $A\subseteq [0,T]$ with $0,T\in A$, let $t_1< t_2< \cdots< t_k$ be the times in $A$. We define $\cten(N,A,T)$ as a classical (steady-state) flow network as follows:
% Here, for $t\in A,t\neq T$ we let $t.succ$ be the smallest value larger than $t$ in the set $A$. Further, let $intervals(A)=\{[t,t.succ)|t\in A\setminus\set{T}\}$ and for any $I=[t,t.succ)$ with $t.succ\neq b$, let $I.succ$ be the interval $[t.succ,(t.succ).succ)$. $t.pred$ and $I.pred$ are defined analogously.
\begin{itemize}
    % \item Define $intervals(A)$ to include the set $[t_i,t_{i+1}-1]$ for all $i=1$ to $k-1$.
    \item The vertex set is $V':=V\times A$.

    \item For all $x\in V$ and all $1\leq j <k$, there is an edge from $(x,t_j)$ to $(x,t_{j+1})$ with infinite capacity.
    % \footnote{Here we use infinity to mean a special (finitely represented) character that is larger than any finite number in comparison. It also works to replace each infinite capacity edge with an edge of capacity larger than the maximum flow (for example, larger than $nUT$, where $U$ is the maximum edge capacity). }
    
    \item For all $xy\in E$ and all $1\leq i,j <k$, there is an edge from $(x,t_i)$ to $(y,t_{j})$ with the following capacity if it is non-zero:
    \begin{align*}
        \sum_{t:(t_i\leq t<t_{i+1}),(t_j\leq t+\tau_{ij} <t_{j+1})}u_{xy}(t).
    \end{align*}

\end{itemize}
Further, we treat $(s,0)$ as the source and $(d,T)$ as the sink. For brevity, we may write $\cten(N,A)$ if $T$ is clear from context.
\end{definition}

Note that $\cten(N,A,T)$ is just $\ten(N,T)$ with all nodes $(v,t)$ for $t\in[t_i,t_{i+1}-1]$ collapsed to a single node $(v,t_i)$, and in fact $\cten(N,[0,T],T)$ is the same as $\ten(N,T)$.
% Note that $\cten(N,[a,b],a,b)$ is the same as $\ten(N,a,b)$, and in general we can view a \cten\ as squeezing together certain intervals of the full \ten\ to form ``meta nodes" and letting the edges between these meta nodes have capacities equal to the sum of the capacities of all edges between  the nodes that made up each meta node. Again, for brevity when we are looking at the interval $[0,T]$ for a choice of $T$ that is clear from context, we will write this as $\cten(N,A)$ and omit the beginning and end of intervals from the notation. 
When $A$ is relatively small, $\cten(N,A)$ can be written much more concisely than $\ten(N)$. In the piecewise constant capacity case, the capacity of new edges can be computed efficiently as well by using multiplication over intervals instead of strictly adding as specified above. 
% Note that $\cten(N,A,T)$ has $|V|\cdot |A|$ nodes.  
% and at most $|A|\cdot  n$ edges. \kristin{verify that this is actually true - need to make sure we're not going to build up a ton of edges via r}
% We already know that the max flow over $[a,b]$ for a time-varying network $N$ has the same value as the classical max flow on $\ten(N)$, but we would like to argue that if $A$ meets certain requirements, then $\cten(N,A)$ also has that same max flow value. Since classical flow networks have the same max flow and min cut value, we will instead compare min cuts of the graphs. 

\subsection*{Finite cuts and cut functions}

% \kristin{resume condensing here}

Cuts are a fundamental tool of flow analysis that we use here, so next we describe cuts on steady-state networks (i.e. networks in which all edge lengths are $0$ and with time horizon $0$). If $N=(V,E)$ is a steady-state network, an $s$-$d$ cut $C$ of $N$ for $s,d\in V$ is a partition of the nodes of $V$ such that $s$ and $d$ are on opposite sides of the partition. The cost of this cut is the collective capacity of edges that go from $s$'s part of the partition (denoted $C(s)$) to $d$'s part of the partition (denoted $C(d)$). A classic result of Ford and Fulkerson \cite{ford1956} states that the minimum cost $s$-$d$ cut on a steady-state network is the same as the maximum $s$-$d$ flow value. Due to the simple structure of cuts, we turn our attention to bounding the values of minimum cuts. 

In the remainder of the paper, we only consider finite capacity cuts. Note that if a steady-state network has an edge $ij$ of infinite capacity, a finite cut $C$ on that steady-state network cannot have $i\in C(s),j\in C(d)$. Crucially, this means that if $N$ is a temporal network, then any finite cut on $\ten(N,T)$ that includes $(i,t)\in C((s,0))$ must also have $(i,t')\in C((s,0))$ for all $t'\geq t$.
We represent finite capacity cuts in a $\ten$ using a {\em cut function} that maps every vertex $i\in V$ to the earliest time $t\in [0,T]$ such that $(i,t)\in C((s,0))$. 
\begin{definition}
    A cut function $\phi$ on $\ten(N,T)$ (or $\cten(N,A,T)$) maps vertices $i\in V$ to the interval $[0,T+1]$ (or to the set $A\cup\set{T+1}$) with $\phi(s)=0$ and $\phi(d)=T+1$, where $s$ is the source and $d$ is the sink. The cut function uniquely represents the $(s,0)$-$(d,T)$ cut $C_\phi$ with $C_\phi((s,0)):=\set{(i,t):i\in V,t\in [0,T],t\geq \phi(i)}$ (or $C_\phi((s,0)):=\set{(i,t):i\in V,t\in A,t\geq \phi(i)}$). We let $cost(\phi)$ be the cost of the cut defined by $C_\phi((s,0))$.
\end{definition}

% We let $cost(\phi)$ be the cost of the $(s,0)$-$(d,T)$ cut defined by $\phi$. 
Note that finite capacity cuts in a $\cten$ form a subset of finite capacity cuts in a $\ten$, so they form a subset of cut functions for $\ten(N,T)$.
% This implies that for any $N, T$, and $A\subseteq [0,T]$ with $0,T\in A$, the capacity of a min $(s,0)$-$(d,T)$ cut in $\ten(N,T)$ is no larger than the capacity of a min $(s,0)$-$(d,T)$ cut in $\cten(N,A,T)$.  
Our goal is to argue that there is a {\em small} $\cten$ that has the same min cut capacity as the $\ten$. To this end, we focus on identifying the ``critical'' times corresponding to edges crossing a min cut in the $\ten$. For a cut function $\phi$, let $\critcut{\phi}$ denote the range of $\phi$, that is, $\critcut{\phi}:=\{t: \exists i\in V \text{ with } \phi(i)=t\}.$
% \[\critcut{\phi}:=\{t: \exists i\in V \text{ with } \phi(i)=t\}.\] 
The following lemma then follows from the correspondence between cut functions of a $\cten$ and a $\ten$.

\begin{lemma}
\label{lem:criticaltimes}
    Let $\phi$ be a cut function corresponding to a min $(s,0)$-$(d,T)$ cut in $\ten(N,T)$, and let $A\subseteq [0,T]$ be any set with $\critcut{\phi}\cap [0,T]\subseteq A$. Then, any min $(s,0)$-$(d,T)$ cut in $\cten(N,A,T)$ is also a min $s$-$d$ cut in $\ten(N,T)$. In particular, the capacity of the min cut in $\cten(N,A,T)$ is equal to the capacity of the min cut in $\ten(N,T)$. 
\end{lemma}

% Note that it is {\em essential} that $\critcut{\phi}\cap [0,T]\subseteq A$. Consider the network depicted in Figure \ref{fig:basic-ten}. The collapsed nodes in the \cten\ merge nodes representing times between $1$ and $3$, and as a result the min cut value of the condensed network is much larger than that of the full network.


% \begin{figure}
%     \centering
%     % \input{figures/basic_ten}
%     \includegraphics[width=.5\textwidth]{figures/fig1flow.pdf}
%     \caption{The top left depicts temporal network $N$, which consists of 5 nodes and in which each edge has infinite capacity for one time step (specified below the edge) and has zero capacity on all other time steps. On the right, we have a full time extended network of $N$ for the period $[0,4]$, and on the bottom left we have $\cten(N,\set{0,1,4},4)$. All edges in the networks have infinite capacity. Note that $\ten(N,4)$ has a min cut of capacity $0$ (depicted by the gold box), while $\cten(N,\set{0,1,4},4)$ has no finite $(s,0)$-$(d,4)$ cut.   }
%     \label{fig:basic-ten}
% \end{figure}


\subsection*{The critical times of a network}

Having established the basic structure of cuts in a $\ten$, we now identify a small set that contains all of the critical times of {\em some} min cut of $\ten(N,T)$. Such a small set $A$ can then be used to construct a small $\cten$ that captures the min cut capacity of the $\ten$ as per Lemma~\ref{lem:criticaltimes}.
Intuitively, we construct our set of critical times to include all times at which some edge changes capacity, as well as certain ``offset'' times from each such change. The idea is that information about the change in some edge capacity may propagate down a path of nodes in the network, so the offset values should correspond to some possible path length in the network. As we have set $\tau$ to be uniform across all edges, all paths in the network have length $\ell\cdot \tau$ for some $\ell\in [0,n]$. Thus, we define our critical times as follows.

%Next we will define a set of points that are important to a particular network. We will later argue that there must exist a min cut of the full \ten\ that has its critical points as a subset of this new set we define. We also define an extended set of critical points that we will use later on. 


% \kristin{rewrite this definition to have a clearer connection to $\mu$}


\begin{definition} \label{def:forbidden}
Let $N=(V,E,\tau,\set{u_{ij}})$ be a network with piecewise constant $u_{ij}$, and let $\breaks$ be the set of times at which some $u_{ij}$ changes value. Also include $0$, $T$, and $T+1$ in $\breaks$. Then 
\begin{align*}
    \critnet{N}:= \set{\theta \pm \ell\cdot \tau:\theta\in \breaks,\ell\in [0,n]}.
\end{align*}
\end{definition}

As before, we let $\mu_{ij}$ be the number of pieces in $u_{ij}$ and $\mu:=\sum_{ij\in E}\mu_{ij}$.
Note that if $\cT$ is as in Definition \ref{def:forbidden}, $|\cT|\leq O(n\mu)$.
% As an example, consider a network on $n$ nodes such that only one edge ever changes capacity, and it only does so at time $t'$. The critical times of this network would be $\set{0,T}\cup \set{(t'-n\cdot \tau),(t'-(n-1)\cdot \tau ),\ldots,(t'-\tau),t',(t'+\tau),\ldots, (t'+(n-1)\cdot \tau),(t'+n\cdot \tau)}$.  
% In particular, we're including in the set of critical points all times that are equal to a breakpoint of the network and all times that are offset from some breakpoint by an integer combination of the travel times, where the integer multipliers are between $0$ and $n$ and must sum to at most $n$.
% multiple between $0$ and $n-1$ of the travel time from some breakpoint of the network. 
% We assume wlog that $0\in \traveltimes$. Note that the size of $\critnet{N}$ is at most $k\cdot  \Pi_{i\in [f],\tau_i\neq 0}2(n+1)=(2(n+1))^{|\traveltimes\setminus \set{0}|}k$ Note that when $|\traveltimes|$ is a constant, this is polynomial in the size of the input graph. In particular, we will primarily consider networks in which all travel times are either $0$ or some uniform travel time $\tau$. Such networks have $|\critnet{N}|\leq 2(n+1)k$.
We can now state our main technical lemma, which we discuss more in Section \ref{sec:proofs}.
\begin{lemma}
\label{lem:breakpoints}
    For any $\ten(N,T)$ there exists a cut function $\phi$ corresponding to a min $(s,0)$-$(d,T)$ cut with $\critcut{\phi}\subseteq\critnet{N}$.
\end{lemma}

Note that Lemma \ref{lem:breakpoints} combined with Lemma \ref{lem:criticaltimes} implies that the maximum $s$-$d$ flow over $T$ on $N$ is exactly the steady-state maximum flow value on $\cten(N,A,T)$, where $A=\critnet{N}$. 
Using Lemma \ref{lem:breakpoints} and a short argument to bound the size of $\cten(N,A,T)$ (which we give in the full version of this paper), we get our main theorem.

\begin{theorem}
If $N=(V,E,\tau,\set{u_{ij}})$ is a temporal network, piecewise constant edge capacities $u_{ij}$ and a constant and uniform edge length $\tau$ on all edges, Let $\mu_{ij}$ be such that $u_{ij}$ has at most $\mu_{ij}$ pieces. Then the maximum $s$-$d$ flow value on $N$ over time horizon $T$ can be found in time $MF(O(n^2\mu),O(mn\mu))$, where $n=|V|,m=|E|,$ $\mu:=\sum_{ij\in E}\mu_{ij}$, and $MF(n',m')$ is the runtime for a steady-state (classical) max flow algorithm on a network with $n'$ nodes and $m'$ edges.
\end{theorem}


% \kristin{move proof to appendix}



==> short_version/short_intro.tex <==
\section{Introduction}

In this paper, we study the problem of maximum flows over time on temporal networks.
We call network parameters that vary over time {\bf temporal} and parameters that are constant {\bf static}. Temporal networks are networks that contain some temporal parameters, while static networks do not.
{Note that flow problems on static networks \cite{Skutella2009} are different from {\em steady-state} or {\em classical} flow problems (i.e. the traditional flow networks introduced by Ford and Fulkerson \cite{ford1956}), as in the former flow takes time to traverse edges.}
Our primary question is: {\bf Given a temporal network $N$, a source $s$, a sink $d$, and a time horizon $T$ what is the maximum amount of flow that can be moved from $s$ to $d$ over time horizon $T$?} We call this the maximum flow over time problem on temporal networks.
% , and in this paper we restrict our attention to a special type of network where all edges have a single static length $\tau$, and all edge capacity functions are piecewise constant.

In this paper, we consider a special case of the temporal maximum flow problem in which all edges have uniform (the same) and static (unchanging) length and all edge capacities are piecewise constant. We show that this special case can be solved for networks of $n$ nodes, $m$ edges, and $\mu$ total ``pieces'' across all edge capacity functions in time $O(MF(\Theta(n^2\mu),\Theta(mn\mu)))$, where $MF(n',m')$ is the runtime of a steady-state maximum flow algorithm on $n'$ nodes and $m'$ edges. Using the $O(m'n')$ max flow algorithm of Orlin \cite{orlin2013}, we can thus solve this problem in strongly polynomial $O(\mu^2n^3m)$ time, or using the  algorithm of Chen et al. \cite{chen2022}, we can solve the problem  in time $ O(\mu^{1+o(1)}(nm)^{1+o(1)}\cdot \log (nTU))$.
Combining the results \cite{hoppe2000,lee2015sfm,orlin1997,chen2022}, the  feasibility variant problem (checking if a given flow value is feasible) can be solved on networks with general edge lengths in strongly polynomial time $\tilde O(\mu^5)$ or weakly polynomial time $ O(\mu^{3+o(1)}\cdot \log^{O(1)}(TU))$. These techniques can be combined with binary search or parametric search to find the maximum flow value, at a cost of increased runtime.
% \footnote{ Although our algorithm only finds the {\em value} of the temporal maximum flow, and not a particular flow, the temporal-to-static TFP reduction of Hoppe and Tardos \cite{hoppe2000} paired with the quickest transshipment solution of Anapolska et al. \cite{anapolska2025} can be used to find a feasible flow of a specified value (if it exists) in time $\tilde O(\mu^7)$. Our runtimes and the ones we compare them to are specifically for finding the {\em value} of the maximum flow. } 
% Table \ref{tab:maxflow} compares runtimes of different algorithms for this problem.

% \input{tab_maxflowval}

In the regime where $\mu>>n,m$ (i.e. the graph undergoes many changes relative to the number of edges and nodes), we get a better runtime than existing algorithms for the maximum flow problem in both the strongly and weakly polynomial settings. If for example $n,m=O(\mu^{1/4})$, we get runtimes $O(\mu^3)$ and $ O(\mu^{3/2+o(1)}\log(nTU))$.


% Our main novel technical contribution is in defining what we call the condensed Time Extended Network (cTEN) by identifying a set of ``critical points'' in the full time expanded network (TEN). The TEN for a network with time horizon $T$ is a static network on node set $V\times[0,T]$\footnote{In this paper, we use $[a,b]$ for $a\leq b$ to refer to the set $\set{a,a+1,a+2,\ldots,b-1,b}$.} whose maximum flow value is equal to the maximum flow over time $T$ on the original network.  We show that if the original network has uniform edge lengths, there is a small set of times $\cT$ such that the TEN must contain a minimum $(s,0)$-$(d,T)$ cut in which if $(i,t)$ is on $(d,T)$'s side of the cut and $(i,t+1)$ is on $(s,0)$'s side of the cut for any $i\in V$, then $t\in \cT$. By the structure of the TEN, we also have that if the min cut has finite capacity, $(i,t)$ being on $(s,0)$'s side of the cut implies $(i,t+1)$ is also on $(s,0)$'s side of the cut, so this set $\cT$ fully captures the times where a node can ``switch sides'' of the cut. The existence of such a set lets us build the cTEN, which is the same as the standard TEN, except that it groups the nodes of $V\times [0,T]$ into intervals whose start times are in $\cT$, reducing the node set to $V\times \cT$. We show that if $\cT$ is chosen appropriately, the minimum $(s,0)$-$(d,T)$ cut value on the cTEN will be the same as the minimum cut value on the full TEN. Thus, the maximum flow value will also be the same. Then the max flow value can be found using a single steady-state maximum flow call on a network of $O(n^2\mu)$ nodes and $O(\mu nm)$ edges, rather than the multiple calls to minimum cost flow algorithms on networks of $\Theta(\mu)$ nodes and edges used by existing techniques. Further, our single call can directly find the maximum flow  over time value, rather than checking if a given flow value is feasible, so it does not require an extra layer of parametric or binary search to find the optimum. A drawback is that it only works on networks with uniform edge lengths.


==> short_version/short_proofs.tex <==

\section{Finding the value of the max flow}\label{sec:proofs}

In this section we  discuss Lemma~\ref{lem:breakpoints}. Our goal is to show the existence of a min cut $\phi$ in $\ten(N,T)$ with $\critcut{\phi}\cap [0,T]\subseteq \critnet{N}$. 
% At a high level, our argument proceeds as follows: We start with an arbitrary min cut. If it does not satisfy the property we need, we show that we can locally modify it without increasing its capacity.  
We first define the local operation on cuts that allows us to move from one min cut to another. Let $\phi$ denote a cut function in $\ten(N,T)$. We use $X_\phi$ to denote vertices that are mapped to $0$ or $T+1$ in $\phi$: $X_\phi:=\{i\in V: \phi(i)\in\{0,T+1\}\}$. Then for any subset $C\subseteq V\setminus X_\phi$, we can define two variants of the cut function $\phi$ -- one where the assignments to vertices in $C$ move ``up'' and the other where the assignments move ``down''. Formally,
\begin{definition}
    Given a cut function $\phi$ in $\ten(N,T)$ and a set $C\subseteq V\setminus X_\phi$, define the cut functions $\phi_C^+$ and $\phi_C^-$ as follows:
    \begin{itemize}
        \item $\phi_C^+(i) := \phi(i)+1$ for all $i\in C$, and $\phi_C^+(i) := \phi(i)$ otherwise. 
        \item $\phi_C^-(i) := \phi(i)-1$ for all $i\in C$, and $\phi_C^-(i) := \phi(i)$ otherwise. 
    \end{itemize}
\end{definition}


%First, we discuss what it means to shift a subset of points by $1$, using the following definition.

%\begin{definition}
%Let $\phi$ be a min cut function on $\ten(N,a,b)$ and let $C\subseteq V$ such that $i\in C$ implies $\critnode{\phi}{i}\neq a,b$. Then for $i\notin C$, $\phi_C(i,t)=\phi_{-C}(i,t)=\phi(i,t)$ for all $t\in[a,b]$. For $i\in C$, let $t\st$ be $\critnode{\phi}{i}$. Then we have:
%\begin{itemize}
    %\item $\phi_C(i,t\st)=s$ and $\phi(i,t)=\phi_C(i,t)$ for all $t\neq t\st$
    %\item $\phi_C(i,t\st-1)=d$ and $\phi(i,t)=\phi_C(i,t)$ for all $t\neq t\st-1$
%\end{itemize}
%\end{definition}

% \kristin{need to make more clear}
Next we identify properties the set $C$ needs to satisfy to ensure that $\phi_C^+$ and $\phi_C^-$ have the same (minimum) capacity as $\phi$.
% Informally, vertices outside of $C$ define certain ``forbidden'' points of time for vertices in $C$, and for each $i\in C$ we will decide if $\phi_C^+(i)$ and $\phi_C^-(i)$ differ from $\phi(i)$ based on whether or not $\phi(i)$ is in this forbidden set. If $\phi(i)$ is in the forbidden set, we adjust $\phi(i)$ by moving it up one (so it  switches to $s$'s side of the cut later on) or down one (so it switches to $s$'s side of the cut earlier on) in $\phi_C^+$ or $\phi_C^-$, respectively.
% . If the cut function assignment to a vertex in $C$ lands in this forbidden set, then the vertex gets pinned at that value, and we cannot move assignments in C up or down. 
Throughout the rest of this section, 
% let $\tau$ be the static travel time of all edges in the network $N$ and 
let $\cT:=\set{t|\exists ij\in E:u_{ij}(t)\neq u_{ij}(t-1)}\cup\set{0,T,T+1}$.
% let $\traveltimes=\set{0=\tau_1,\tau_2,\ldots,\tau_f}$ be the set of possible travel times for network $N$. In other words, $\tau\in \traveltimes$ for all $ij\in E$.

%Note that in the above definition, $\critnode{\phi}{i}+1=\critnode{\phi_C}{i}$ for all $i\in C$ (and is unchanged for $i\notin C$) and $\critnode{\phi}{i}-1=\critnode{\phi_{-C}}{i}$  for $i\in C$. 
%First we will argue a property about $\phi,\phi_C,$ and $\phi_{-C}$.

\begin{definition}
Given a cut function $\phi$ in $\ten(N,T)$, a set $C\subseteq V\setminus X_\phi$, and some vertex $i\in C$, define $\forbidden{\phi}{C}{i}$ as the union of the following sets: 
\begin{itemize}
        \item $\breaks\cup\{\theta+\tau : \theta\in\breaks\}$ 
        \item $\{\phi(j)-\tau,\phi(j) : ij\in E \text{ and } j\in V\setminus C\}$ 
        \item $\{\phi(j)+\tau,\phi(j) : ji\in E \text{ and } j\in V\setminus C\}$ 
\end{itemize}
%Further, $\forbidden{\phi}{}{i}$ is defined as $\forbidden{\phi}{\set{i},i}$.
\end{definition}


In the full version of the paper, we prove Claim \ref{lem:local-op}, which states that if $\phi(i)$ does not fall into one of the ``forbidden'' points for $(i,\phi,C)$, then $\phi_C^+$ and $\phi_C^-$ have the same cost as $\phi$. 

\begin{claim}
\label{lem:local-op}
    Given a network $N$ and min $s$-$d$ cut function $\phi$, let $C\subseteq V\setminus X_\phi$ satisfy $\phi(i)\notin \forbidden{\phi}{C}{i}$ for all $i\in C$. Then $cost(\phi_C^+)=cost(\phi_{C}^-)=cost(\phi)$.
\end{claim}

\begin{figure}
    \centering
    % \input{figures/bad_edge_in}
    % \input{figures/bad_edge_out}
    \includegraphics[width=.48\textwidth]{figures/fig2aflow.pdf}
    % \includegraphics[width=.48\textwidth]{figures/fig2bflow.pdf}
    \caption{
    % This figure provides a visualization of why certain points are forbidden when trying to shift $\phi$ up or down. In this example, the travel time is $1$, and green nodes are on $(s,0)$'s side of the cut, and red nodes are on $(d,T)$'s side. Thus, the edges that incur a cost for this cut are edges that go from green to red.   \\
    This figure depicts a problem with edge cancellation in the proof of Claim \ref{lem:local-op} when there exists $i\in C$ and  $j\in V\setminus C$ with $\phi(i)=\phi(j)+\tau$. In particular for this graph, $\movedown{C}$ incurs an extra cost for edge $(i,\phi(i)-1)(j,\phi(j)-1)$ but $\moveup{C}$ does not incur an equivalent discount for the edge $(i,\phi(i))(j,\phi(j))$, as this edge was already free under $\phi$.
    % \\
    % Subfigure (b) depicts a problem with edge cancellation in the proof of Claim \ref{lem:local-op} when there exists $i\in V\setminus C$ and $j\in C$ with $\phi(i)=\phi(j)+\tau$. In particular, for this graph $\moveup{C}$ incurs an extra cost for the edge $(i,\phi(i))(j,\phi(j))$ but $\moveup{C}$ does not incur an equivalent discount for the edge $(i,\phi(i)-1)(j,\phi(j)-1)$, as this edge was already free under $\phi$.
    }
    \label{fig:bad-edges}
\end{figure}


We briefly outline the idea of this claim. Note that some number of copies of each edge $ij\in E$ crosses the cut defined by $\phi$. We want to show that if $\phi_C^+$ incurs some additional cost by having an extra copy of $ij$ cross it as compared to $\phi$, then $\phi_C^-$ obtains an equivalent ``discount'' by having one less copy of $ij$ cross it as compared to $\phi$. The reverse is also true -- that is $\phi_C^+$ gets a total discount value equal to the total extra cost value of $\phi_C^-$. As neither $\phi_C^+$ nor $\phi_C^-$ can be cheaper than $\phi$, it must be the case that all three cuts have the same cost. Figure \ref{fig:bad-edges} discusses an example of how these costs and discounts might offset.

Given Claim \ref{lem:local-op}, we can prove Lemma \ref{lem:breakpoints} by considering a min cut function $\phi$ that maximizes $\sum_{i\in V}\phi(i)$. If there is a node $i$ such that $\phi(i)$ is not offset by a factor of $\tau$ of some $\theta\in \cT$, we define $C$ to be $i$ and all of the nodes $j$ such that $\phi(j)$ is offset by a factor of $i$ from $\phi(i)$, and we show that $C$ meets the criteria of Claim \ref{lem:local-op}, so $\moveup{C}$ is a min cut with higher sum of $\phi(i)$ values. Then we show that if  $\critcut{\phi}\cap [0,T]\not\subseteq \critnet{N}$, there exists an $i\in V$ such that $\phi(i)$ is not offset from any $\theta\in \cT$ by a multiple of $\tau$, so $\phi$ cannot be a min cut function maximizing $\sum_{i\in V}\phi(i)$.
The full proof of the lemma is in the full version of this paper.

% To give some intuition for the offsetting discounts and extra costs, note that the number of ``copies'' of $ij$ that cross the cut $\phi$ is at most $\max\set{0,\Delta_{ij}^\phi}$, where $\Delta_{ij}^\phi:=\phi(j)-(\phi(i)+\tau)$. If $i,j\in C$ or $i,j\in V\setminus C$, $\Delta_{ij}^\phi=\Delta_{ij}^{\phi_C^+}=\Delta_{ij}^{\phi_C^-}$, as $\phi(i)$ and $\phi(j)$ change by the same amount.
% % $\phi(i)$ and $\phi(j)$ change by the same amount under $\phi_C^+$ and $\phi_C^-$, so the extra costs associated with one change should equal the discounts associated with the other change. 
% Alternatively, consider the case that $i\in C,j\in V\setminus C$. We have $\Delta_{ij}^{\phi_C^-}=\phi(j)-(\phi(i)-1+\tau)=\Delta_{ij}^\phi+1$. Likewise, $\Delta_{ij}^{\phi_C^+}=\Delta_{ij}^\phi-1$. Thus, if $\max\set{0,\Delta_{ij}^{\phi_C^+}}-\max\set{0,\Delta_{ij}^{\phi}}\neq \max\set{0,\Delta_{ij}^{\phi}}-\max\set{0,\Delta_{ij}^{\phi_C^-}} $ (i.e. the extra cost incurred by $\phi_C^+$ for this edge is not equal to the extra discount incurred by $\phi_C^-$), then we have $\max\set{0,\Delta_{ij}^\phi+1}-\max\set{0,\Delta_{ij}^\phi}\neq \max\set{0,\Delta_{ij}^\phi}-\max\set{0,\Delta_{ij}^\phi-1}$, which implies that $0=\Delta_{ij}^\phi=\phi(j)-(\phi(i)+\tau)$ (as $\Delta_{ij}^\phi$ must be an integer). However, since $j\in C$ and $ij\in E$, $\phi(j)-\tau$ is a forbidden point for $\phi(i)$ and this is impossible. Figure \ref{fig:bad-edges} gives a visual sense of this phenomenon, and the proof of Claim \ref{lem:local-op} at the end of the section gives a full and more  careful analysis.

% Recalling that $\phi_C^+(j)=\phi_C^-(j)=\phi(j)$ and $\phi_C^+(i)=\phi(i)+1,\phi_C^-(i)=\phi(i)-1$, we have that  if $(\max\set{0,\phi(j)-(\phi(i)-\tau))}-\max\set{0,\phi_C^+(j)-(\phi_C^+(i)-\tau))})<0$ (i.e. $\phi_C^+$ incurs an extra cost for edge $ij$), then  $\phi(j)-(\phi(i)+1+\tau)>\phi(j)-(\phi(i)+\tau)\implies \phi(j)$

% consider an edge $ij\in E$ where at least one copy of $ij$ crosses the cut defined by $\phi$ (i.e. $\phi(j)>\phi(i)+\tau$). If both $i,j\in C$ or both $i,j\notin C$, both 


% In particular, we want to show that if $\phi_C^+$ gets some extra cost for moving $\phi(i)$ up, then $\phi_C^-$ should get the same amount as a ``discount'' for moving $\phi(i)$ down. That is, if $\phi_C^+(i)$ incurs some extra cost, there must exist some edge $ji$ such that $(j,\phi(i)+1-\tau)(i,\phi(i)+1)$ is an edge that crosses the new cut. However, this implies that $\phi_C^+(j)\leq \phi(i)+1-\tau$. If $\phi_C^-(j)=\phi(i)+1-\tau$, it must be the case that 
% Since neither $\phi_C^-$ nor $\phi_C^+$ can be cheaper than $\phi$, it must be the case that  all three cuts have equal cost.







% We are now ready to describe an algorithm for obtaining a min cut $\phi$ in the $\ten$ that satisfies $\critcut{\phi}\subseteq \critnet{N}$, thus proving Lemma \ref{lem:breakpoints}. In every iteration our algorithm finds a subset $C$ of vertices that satisfies the assumption in Claim~\ref{lem:local-op}, namely that $\phi(i)\not\in\forbidden{\phi}{C}{i}$ for all $i\in C$. If such a subset exists, we can change the cut to $\phi := \phi_C^+$ while maintaining minimum capacity. On the other hand, if no such set exists, we show that the cut function assignment to each vertex, $\phi(i)$, is ``pinned'' to a value in $\critnet{N}$, proving the property we need. 
% We keep track of pinned assignments by defining an auxiliary graph on vertices and breakpoints as follows. 

% %To argue that $\critcut{\phi\st}\subseteq \critnetoff{N}$ for some min cut $\phi\st$, we will take an arbitrary min cut $\phi$ on $\ten(N,a,b)$ and ``shift'' it to define a new min cut on $\ten(N,a,b)$ with the desired properties. To do this, we give Algorithm \ref{alg:shift} and prove that the output has the desired properties. 


% Now we define auxillary graphs $G_\phi$ for each min cut $\phi$ that will help us in our proof. 

% \begin{definition}
%     The {\em pinned assignments graph} $G_\phi$ for $\ten(N,T)$ is an unweighted undirected graph on $V\cup \breaks$ with an edge set defined as follows: 
%     % The graph is {\em compatible} with a cut function $\phi$ if it satisfies the following properties:
%     \begin{itemize}
%         \item Any edge $\set{i,j}$ is in $G_\phi$ for $i,j\in V$ iff $|\phi(i)-\phi(j)|\in \set{0,\tau}$.
%         \item An edge $\set{i,\theta}$ is in $G_\phi$ for $i\in V$ and $\theta\in\breaks$ iff $|\phi(i)-\theta|\in \set{0,\tau}$.
%     \end{itemize}
% \end{definition}


